Preventing Your Faults From Telling Your Secrets: Defenses Against Pigeonhole Attacks

New hardware primitives such as Intel SGX secure a user-level process in presence of an untrusted or compromised OS. Such "enclaved execution" systems are vulnerable to several side-channels, one of which is the page fault channel. In this paper, we show that the page fault side-channel has sufficient channel capacity to extract bits of encryption keys from commodity implementations of cryptographic routines in OpenSSL and Libgcrypt --- leaking 27% on average and up to 100% of the secret bits in many case-studies. To mitigate this, we propose a software-only defense that masks page fault patterns by determinising the program's memory access behavior. We show that such a technique can be built into a compiler, and implement it for a subset of C which is sufficient to handle the cryptographic routines we study. This defense when implemented generically can have significant overhead of up to 4000X, but with help of developer-assisted compiler optimizations, the overhead reduces to at most 29.22% in our case studies. Finally, we discuss scope for hardware-assisted defenses, and show one solution that can reduce overheads to 6.77% with support from hardware changes.

==> tables/information_flow_types.tex <==
\begin{table*}
\centering
\caption{Information flow analysis for our language defined in Figure ~\ref{fig:grammar}. Label $\mathit{l}$() represents sensitivity of each statement.}
\label{tbl:transforms}

\resizebox{\textwidth}{!}{%

\begin{tabular}{|l|ll|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{{\bf Grammar Terms}}                                    & \multicolumn{1}{c|}{{\bf Grammar Rule}}                          & \multicolumn{5}{l|}{{\bf Inferred Label}}                                                                                                                     \\ \hline
Program                       & S                     & ::=                  & \texttt{begin_pf_sensitive} P \texttt{end_pf_sensitive}          & \multicolumn{5}{l|}{$\mathit{l}$(P) $\leftarrow$ \texttt{high}}                                                                                                          \\ \hline
\multirow{7}{*}{Commands}     & \multirow{7}{*}{P}    & \multirow{7}{*}{::=} & lval = e                                                         & \multicolumn{5}{l|}{$\mathit{l}$(lval) $\leftarrow$ $\mathit{l}$(P),  $\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(P)}                                                                                       \\ \cline{4-9} 
                              &                       &                      & \texttt{if} (e) \texttt{then} P else P'                          & \multicolumn{5}{l|}{$\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(P) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(P') $\leftarrow$ $\mathit{l}$(P)}                                                                  \\ \cline{4-9} 
                              &                       &                      & \texttt{do} \{P\} \texttt{while} ($\lceil$e$\rceil^{c}$)         & \multicolumn{5}{l|}{$\mathit{l}$(P) $\leftarrow$ $\mathit{l}$(P) , $\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(c) $\leftarrow$ $\mathit{l}$(P)}                                                                  \\ \cline{4-9} 
                              &                       &                      & \texttt{while} ($\lceil$e$\rceil^{c}$) do \{P\}                  & \multicolumn{5}{l|}{$\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(c) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(P) $\leftarrow$ $\mathit{l}$(P)}                                                                   \\ \cline{4-9} 
                              &                       &                      & \texttt{for} (e$_{1}$; $\lceil$e$_{2}$$\rceil^{c}$; e$_{3}$) {P} & \multicolumn{5}{l|}{$\mathit{l}$(e$_{1}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(e$_{2}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(c) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(e$_{3}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(P) $\leftarrow$ $\mathit{l}$(P)} \\ \cline{4-9} 
                              &                       &                      & f (e$_{1}$, e$_{2}$, $\mathellipsis$, e$_{n}$) \{P\}             & \multicolumn{5}{l|}{$\mathit{l}$(e$_{1}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(e$_{2}$) $\leftarrow$ $\mathit{l}$(P), $\mathellipsis$, $\mathit{l}$(e$_{n}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(P) $\leftarrow$ $\mathit{l}$(P)}        \\ \cline{4-9} 
                              &                       &                      & \texttt{return} e                                                & \multicolumn{5}{l|}{$\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(P)}                                                                                                                   \\ \hline
\multirow{10}{*}{Expressions} & \multirow{7}{*}{e}    & \multirow{7}{*}{::=} & e$_{1}$ $\oslash$ e$_{2}$                                        & \multicolumn{5}{l|}{$\mathit{l}$(e$_{1}$) $\leftarrow$ $\mathit{l}$(e), $\mathit{l}$(e$_{2}$) $\leftarrow$ $\mathit{l}$(e)}                                                                               \\ \cline{4-9} 
                              &                       &                      & e$_{1}$ ? e$_{2}$ : e$_{3}$                                      & \multicolumn{5}{l|}{$\mathit{l}$(e$_{1}$) $\leftarrow$ $\mathit{l}$(e), $\mathit{l}$(e$_{2}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(e$_{3}$) $\leftarrow$ $\mathit{l}$(e)}                                                 \\ \cline{4-9} 
                              &                       &                      & $\circledcirc$ e                                                 & \multicolumn{5}{l|}{$\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(e)}                                                                                                                   \\ \cline{4-9} 
                              &                       &                      & $\odot$ lval                                                     & \multicolumn{5}{l|}{$\mathit{l}$(lval) $\leftarrow$ $\mathit{l}$(e)}                                                                                                                \\ \cline{4-9} 
                              &                       &                      & lval                                                             & \multicolumn{5}{l|}{$\mathit{l}$(lval) $\leftarrow$ $\mathit{l}$(e)}                                                                                                                \\ \cline{4-9} 
                              &                       &                      & c                                                                & \multicolumn{5}{l|}{$\mathit{l}$(c) $\leftarrow$ $\mathit{l}$(e)}                                                                                                                   \\ \cline{4-9} 
                              &                       &                      & foo (e$_{1}$, e$_{2}$, $\mathellipsis$, e$_{n}$)                 & \multicolumn{5}{l|}{$\mathit{l}$(e$_{1}$) $\leftarrow$ $\mathit{l}$(P), $\mathit{l}$(e$_{2}$) $\leftarrow$ $\mathit{l}$(P), $\mathellipsis$, $\mathit{l}$(e$_{n}$) $\leftarrow$ $\mathit{l}$(P)}                                \\ \cline{2-9} 
                              & c                     & ::=                  & \texttt{const}                                                   & \multicolumn{5}{l|}{$\mathit{l}$(\texttt{const}) $\leftarrow$ \texttt{low}}                                                                                              \\ \cline{2-9} 
                              & \multirow{2}{*}{lval} & \multirow{2}{*}{::=} & \texttt{var}                                                     & \multicolumn{5}{l|}{$\mathit{l}$(\texttt{var}) $\leftarrow$ $\mathit{l}$(lval)}                                                                                                     \\ \cline{4-9} 
                              &                       &                      & \texttt{var} [e]                                                 & \multicolumn{5}{l|}{$\mathit{l}$(\texttt{var}) $\leftarrow$ $\mathit{l}$(lval), $\mathit{l}$(e) $\leftarrow$ $\mathit{l}$(lval)}                                                                          \\ \hline
\end{tabular}
}
\end{table*}
% \vspace{-.10cm}


==> tables/stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\label{tab:stats}
\centering
% \resizebox{\textwidth}{!}{%

\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|r|r|r|}
\hline
\multicolumn{1}{|l|}{\multirow{4}{*}{{\bf Library}}}                          & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf Cases}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf \begin{tabular}[c]{@{}c@{}}Sensitive \\ Functions\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf \begin{tabular}[c]{@{}c@{}}Basic \\ Blocks\end{tabular}}}} & \multicolumn{3}{c|}{\multirow{2}{*}{{\bf Basic Block  Size}}}                                                                                       & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf Loops}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf \begin{tabular}[c]{@{}c@{}}Sensitive \\ Variables\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf LoC}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf \begin{tabular}[c]{@{}c@{}}Staging\\ Area \\ (Pages)\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf \begin{tabular}[c]{@{}c@{}}Runtime calls\\ to Sensitive \\ Functions\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{4}{*}{{\bf \begin{tabular}[c]{@{}c@{}}Total Runtime\\ MUX Accesses\end{tabular}}}} \\
\multicolumn{1}{|l|}{}                                                        & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{}                                                                               & \multicolumn{3}{c|}{}                                                                                                                               & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                                                                                         & \multicolumn{1}{c|}{}                                                                                                         & \multicolumn{1}{c|}{}                                                                                            \\ \cline{5-7}
\multicolumn{1}{|l|}{}                                                        & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{}                                                                               & \multicolumn{1}{l|}{\multirow{2}{*}{{\bf Min}}} & \multicolumn{1}{l|}{\multirow{2}{*}{{\bf Max}}} & \multicolumn{1}{l|}{\multirow{2}{*}{{\bf Avg}}} & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                                                                                         & \multicolumn{1}{c|}{}                                                                                                         & \multicolumn{1}{c|}{}                                                                                            \\
\multicolumn{1}{|l|}{}                                                        & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{}                                                                               & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                                                                                         & \multicolumn{1}{c|}{}                                                                                                         & \multicolumn{1}{c|}{}                                                                                            \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Libgcrypt\\ (v1.6.3)\end{tabular}} & AES                                               & 1                                                                                                          & 1                                                                                                   & 248                                             & 248                                             & 248                                             & 0                                                 & 22                                                                                                         & 272                                             & 3                                                                                                             & 1                                                                                                                             & 112                                                                                                              \\ \cline{2-13} 
                                                                              & \cast                                             & 1                                                                                                          & 1                                                                                                   & 940                                             & 940                                             & 940                                             & 0                                                 & 11                                                                                                         & 47                                              & 3                                                                                                             & 2                                                                                                                             & 320                                                                                                              \\ \cline{2-13} 
                                                                              & EdDSA                                             & 31                                                                                                         & 701                                                                                                 & 1                                               & 39                                              & 6                                               & 56                                                & 178                                                                                                        & 1212                                            & 2                                                                                                             & 1                                                                                                                             & 60725                                                                                                            \\ \cline{2-13} 
                                                                              & \powm                                             & 20                                                                                                         & 297                                                                                                 & 1                                               & 36                                              & 6                                               & 47                                                & 126                                                                                                        & 796                                             & 2                                                                                                             & 1                                                                                                                             & 57660                                                                                                            \\ \cline{2-13} 
                                                                              & SEED                                              & 1                                                                                                          & 11                                                                                                  & 2                                               & 63                                              & 12                                              & 1                                                 & 17                                                                                                         & 56                                              & 3                                                                                                             & 1                                                                                                                             & 128                                                                                                              \\ \cline{2-13} 
                                                                              & Stribog                                           & 1                                                                                                          & 1                                                                                                   & 418                                             & 418                                             & 418                                             & 0                                                 & 5                                                                                                          & 31                                              & 5                                                                                                             & 250                                                                                                                           & 2000                                                                                                             \\ \cline{2-13} 
                                                                              & Tiger                                             & 1                                                                                                          & 1                                                                                                   & 60                                              & 60                                              & 60                                              & 0                                                 & 12                                                                                                         & 18                                              & 3                                                                                                             & 312                                                                                                                           & 2496                                                                                                             \\ \cline{2-13} 
                                                                              & Whirlpool                                         & 1                                                                                                          & 3                                                                                                   & 48                                              & 683                                             & 287                                             & 1                                                 & 16                                                                                                         & 112                                             & 6                                                                                                             & 6                                                                                                                             & 7680                                                                                                             \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}OpenSSL\\ (v1.0.2)\end{tabular}}   & \cast                                             & 1                                                                                                          & 12                                                                                                  & 3                                               & 746                                             & 79                                              & 4                                                 & 14                                                                                                         & 93                                              & 3                                                                                                             & 1                                                                                                                             & 160                                                                                                              \\ \cline{2-13} 
                                                                              & SEED                                              & 1                                                                                                          & 1                                                                                                   & 948                                             & 948                                             & 948                                             & 0                                                 & 13                                                                                                         & 58                                              & 3                                                                                                             & 1                                                                                                                             & 128                                                                                                              \\ \hline
\end{tabular}
% 
% \vspace{-1cm}
\caption{Analysis Summary. Column 4 denotes the number of execution blocks in the sensitive portion. Columns 5, 6 and 7 denote the mininum, maximum and average size (in number of instruction count) of the execution blocks. Column 11 gives the number pages allocated for staging area instances. Column 13 gives the total number of accesses to the staging area at runtime.}
% \vspace{-.3cm}
\end{table}
